Asymptotic safety of gravity with matter

The asymptotic-safety paradigm posits that the symmetry of quantum theories of gravity and matter is enhanced to quantum scale symmetry, i.e., scale symmetry in the presence of quantum fluctuations, at very high energies. To achieve such a symmetry enhancement, the effect of quantum fluctuations must balance out. It is to be expected that such a balance can only be achieved within a set of theories with limited field content and interaction structure. In this chapter, we review how much is known about these limits. From the quantum scale invariant regime, the theory transits to a theory with distinct physical scales - most importantly masses for various elementary particles - at low energies. There, quantum scale invariance can leave its imprint in relations between various interactions and mass scales of the theory. These relations can be compared to experimental data, which has two possible implications: first, if the relations do not match the data, the underlying quantum theory of gravity and matter, formulated at and beyond the Planck scale, has been ruled out using experimental data from energies much below the Planck scale. Second, if the relations match the data, the asymptotic-safety paradigm provides a first-principles derivation of free parameters of the Standard Model. Most importantly, this may include the ratios of the Higgs mass to the electroweak scale as well as the value of the finestructure constant. Similarly, theories beyond the Standard Model may come with fewer free parameters than in their effective-field-theory incarnation without gravity. This may lead to an explanation of the smallness of neutrinos masses and predictions for the nature and interactions of dark matter.

==> Input/Scalarsincosmo.tex <==
\colMS{\bf[MS: moved Higgs inflation to further reading in Higgs sector, commented out rest of the section here.]}
%\subsection{Inflation}
%\subsubsection{Higgs inflation}
%\emph{Synopsis: Higgs inflation, which can explain inflation without the need for extra fields beyond the SM, appears to be incompatible with asymptotically safe gravity.}
%Higgs inflation \cite{} is based on a nonminimal coupling $\xi$ between the Higgs scalar and the curvature scalar. A change to the Einstein-frame, i.e., a conformal transformation of the metric that removes the nonminimal coupling, produces a potential that is appropriate for inflation for suitable values of the couplings. This model is attractive due to its predictive power, because it does not require any BSM fields and contains only one free parameter, namely the nonminimal coupling. In \cite{Eichhorn:2020kca}, it was found that the nonminimal coupling is predicted in asymptotic safety, at least for those values of $G$ and $\Lambda$, for which Yukawa couplings can be nonzero. It turns out that the predicted ratio $\lambda_4/\xi^2$ between the Higgs quartic coupling and the nonminimal coupling is much too large to be compatible with CMB data. This result, if confirmed in extended truncations, rules out Higgs inflation in asymptotically safe gravity. The same conclusion was achieved already in \cite{Wetterich:2019rsn}, based on a study of the Higgs potential at large field values.
%
%\subsection{Inflaton}
%
%\subsection{Dynamical dark energy}
